Supervised and Unsupervised Neural Network Solver for First Order Hyperbolic Nonlinear PDEs

We present a neural network-based method for learning scalar hyperbolic conservation laws. Our method replaces the traditional numerical flux in finite volume schemes with a trainable neural network while preserving the conservative structure of the scheme. The model can be trained both in a supervised setting with efficiently generated synthetic data or in an unsupervised manner, leveraging the weak formulation of the partial differential equation. We provide theoretical results that our model can perform arbitrarily well, and provide associated upper bounds on neural network size. Extensive experiments demonstrate that our method often outperforms efficient schemes such as Godunov's scheme, WENO, and Discontinuous Galerkin for comparable computational budgets. Finally, we demonstrate the effectiveness of our method on a traffic prediction task, leveraging field experimental highway data from the Berkeley DeepDrive drone dataset.

==> figs/2d_final_density/burgers_godunov.tex <==
-0.45774102210998535
-0.47943851351737976
-0.47944551706314087
-0.48079714179039
-0.4836008846759796
-0.48789024353027344
-0.4935864806175232
-0.5004717707633972
-0.5081896185874939
-0.5162827372550964
-0.524261474609375
-0.5316821336746216
-0.5382095575332642
-0.5436459183692932
-0.5479251742362976
-0.5510857105255127
-0.5532329678535461
-0.5545059442520142
-0.5550516247749329
-0.5550099611282349
-0.5545051097869873
-0.5536442399024963
-0.5525172352790833
-0.5512006878852844
-0.549760103225708
-0.54825359582901
-0.5467346906661987
-0.5452549457550049
-0.543864905834198
-0.5426169633865356
-0.541565477848053
-0.5407683849334717
-0.5402880311012268
-0.5401911735534668
-0.5405497550964355
-0.5414406061172485
-0.5429450273513794
-0.5451481342315674
-0.5481379628181458
-0.5520070195198059
-0.5568524599075317
-0.5627801418304443
-0.5699069499969482
-0.5783600211143494
-0.5882648825645447
-0.5997158288955688
-0.612724781036377
-0.6271573305130005
-0.6426756381988525
-0.6587234139442444
-0.6745782494544983
-0.6894657015800476
-0.7026978135108948
-0.7137826681137085
-0.7224709987640381
-0.7287393808364868
-0.7327324151992798
-0.734694242477417
-0.734909176826477
-0.7336596250534058
-0.7312024831771851
-0.7277581691741943
-0.7235094904899597
-0.7186033725738525
-0.7131569385528564
-0.7072619795799255
-0.7009904384613037
-0.6943991780281067
-0.6875326037406921
-0.6804261207580566
-0.6731081604957581
-0.6656022071838379
-0.6579273343086243
-0.6500999331474304
-0.6421336531639099
-0.6340402364730835
-0.6258305907249451
-0.6175135970115662
-0.6090975403785706
-0.6005899906158447
-0.5919974446296692
-0.5833262205123901
-0.5745815634727478
-0.565768837928772
-0.5568927526473999
-0.5479573011398315
-0.5389665961265564
-0.5299242734909058
-0.5208334922790527
-0.5116972923278809
-0.5025185346603394
-0.4932998716831207
-0.48404353857040405
-0.4747517704963684
-0.46542659401893616
-0.4560699164867401
-0.44668352603912354
-0.4372687339782715
-0.4278271794319153
-0.4183601438999176
-0.40886878967285156
-0.39935430884361267
-0.3898176848888397
-0.3802599012851715
-0.3706817328929901
-0.3610839247703552
-0.35146719217300415
-0.34183233976364136
-0.3321796655654907
-0.3225097060203552
-0.3128229081630707
-0.30311962962150574
-0.2934001088142395
-0.2836645245552063
-0.27391350269317627
-0.26414796710014343
-0.2543729543685913
-0.24461019039154053
-0.2349601536989212
-0.22590012848377228
-0.2197335809469223
-0.22702603042125702
-0.28283077478408813
-0.4228406846523285
-0.5822409391403198
-0.6783977150917053
-0.7177808284759521
-0.7310693264007568
-0.7351173758506775
-0.7362599968910217
-0.7365548610687256
-0.7366196513175964
-0.736627995967865
-0.7366251349449158
-0.7366217374801636
-0.736619770526886
-0.7366188764572144
-0.7366185188293457
-0.736618161201477
-0.7366177439689636
-0.736617386341095
-0.7366170287132263
-0.7366166114807129
-0.7366162538528442
-0.7366158962249756
-0.7366154789924622
-0.7366151213645935
-0.7366147637367249
-0.7366143465042114
-0.7366139888763428
-0.7366136312484741
-0.7366132140159607
-0.736612856388092
-0.7366124987602234
-0.73661208152771
-0.7366117238998413
-0.7366113662719727
-0.7366109490394592
-0.7366105914115906
-0.7366102337837219
-0.7366098165512085
-0.7366094589233398
-0.7366091012954712
-0.7366086840629578
-0.7366083264350891
-0.7366079688072205
-0.736607551574707
-0.7366071939468384
-0.7366068363189697
-0.7366064190864563
-0.7366060614585876
-0.736605703830719
-0.7366052865982056
-0.7366049289703369
-0.7366045713424683
-0.7366041541099548
-0.7366037964820862
-0.7366034388542175
-0.7366030216217041
-0.7366026639938354
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668

==> figs/2d_final_density/burgers_lax_hopf.tex <==
-0.45774102210998535
-0.45774102210998535
-0.45774102210998535
-0.45774102210998535
-0.45774102210998535
-0.45774102210998535
-0.45774102210998535
-0.45774102210998535
-0.46310532093048096
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5650272369384766
-0.5643375515937805
-0.5558617115020752
-0.5458416938781738
-0.5358407497406006
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.531444787979126
-0.573819100856781
-0.6020686626434326
-0.6020686626434326
-0.6020686626434326
-0.6020686626434326
-0.6020686626434326
-0.6020686626434326
-0.6669842600822449
-0.7875418663024902
-0.7875418663024902
-0.7875418663024902
-0.7875418663024902
-0.7875418663024902
-0.7875418663024902
-0.7875418663024902
-0.7875418663024902
-0.7875418663024902
-0.7875418663024902
-0.785688042640686
-0.7763025760650635
-0.7662825584411621
-0.7562625408172607
-0.7462424635887146
-0.7362224459648132
-0.7262023687362671
-0.7161823511123657
-0.7061623334884644
-0.6961422562599182
-0.6861222386360168
-0.6761022210121155
-0.6660821437835693
-0.656062126159668
-0.6460420489311218
-0.6360220313072205
-0.6260020136833191
-0.615981936454773
-0.6059619188308716
-0.5959419012069702
-0.5859218239784241
-0.5759018063545227
-0.5658817291259766
-0.5558617115020752
-0.5458416938781738
-0.5358216166496277
-0.5258015990257263
-0.515781581401825
-0.5057615041732788
-0.49574148654937744
-0.4857214391231537
-0.47570139169692993
-0.4656813442707062
-0.4556613266468048
-0.44564127922058105
-0.4356212317943573
-0.42560118436813354
-0.4155811667442322
-0.4055611193180084
-0.39554107189178467
-0.3855210244655609
-0.37550100684165955
-0.3654809594154358
-0.35546091198921204
-0.3454408645629883
-0.3354208469390869
-0.32540079951286316
-0.3153807520866394
-0.30536070466041565
-0.2953406870365143
-0.2853206396102905
-0.2753005921840668
-0.265280544757843
-0.25526052713394165
-0.2452404797077179
-0.23522043228149414
-0.22520039975643158
-0.21518035233020782
-0.20516031980514526
-0.1951402723789215
-0.18512023985385895
-0.1751001924276352
-0.16508015990257263
-0.5342023372650146
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668

==> figs/2d_final_density/burgers_ours.tex <==
-0.45774102210998535
-0.4582466781139374
-0.4558110237121582
-0.4572593569755554
-0.45728600025177
-0.4553866982460022
-0.4538269639015198
-0.4621604382991791
-0.5089184641838074
-0.5654846429824829
-0.5688460469245911
-0.5586079359054565
-0.5606938600540161
-0.5655419826507568
-0.5664201378822327
-0.5646724700927734
-0.5644850134849548
-0.5655477643013
-0.5663246512413025
-0.566415548324585
-0.5656936168670654
-0.5637683868408203
-0.5602989196777344
-0.5554412603378296
-0.5497300624847412
-0.5438209772109985
-0.5384002327919006
-0.5341664552688599
-0.5316975116729736
-0.5311172604560852
-0.5317673087120056
-0.5324462056159973
-0.5323379039764404
-0.5316481590270996
-0.531154215335846
-0.5312881469726562
-0.5317276120185852
-0.5317777991294861
-0.5306835770606995
-0.5283282995223999
-0.5269124507904053
-0.5316675305366516
-0.5538604855537415
-0.5894404649734497
-0.6051663756370544
-0.6012213826179504
-0.5944682955741882
-0.5921649932861328
-0.5907291173934937
-0.6257917881011963
-0.7509161233901978
-0.7776041030883789
-0.7762619256973267
-0.7833755016326904
-0.7850922346115112
-0.7933224439620972
-0.7922765612602234
-0.7940557599067688
-0.7906887531280518
-0.7874458432197571
-0.7816678285598755
-0.775099515914917
-0.7676545977592468
-0.7593526244163513
-0.7508342266082764
-0.7417188286781311
-0.7325276136398315
-0.7230558395385742
-0.7134658694267273
-0.7037999033927917
-0.6940213441848755
-0.6842177510261536
-0.6743701696395874
-0.6644889116287231
-0.6545915007591248
-0.6446775794029236
-0.6347544193267822
-0.6248252391815186
-0.6148918867111206
-0.60495525598526
-0.5950173139572144
-0.5850785374641418
-0.5751399397850037
-0.5652014017105103
-0.5552634596824646
-0.5453248620033264
-0.5353848934173584
-0.5254440903663635
-0.5155029296875
-0.5055606961250305
-0.49561694264411926
-0.48567184805870056
-0.4757240414619446
-0.46577394008636475
-0.45582157373428345
-0.44586601853370667
-0.4359075129032135
-0.4259457588195801
-0.41598063707351685
-0.40601176023483276
-0.3960387408733368
-0.3860625922679901
-0.37608230113983154
-0.3660980463027954
-0.3561100959777832
-0.34611833095550537
-0.33612316846847534
-0.3261245787143707
-0.3161216378211975
-0.30611535906791687
-0.2961060404777527
-0.28609392046928406
-0.2760770916938782
-0.26606103777885437
-0.256033718585968
-0.24602270126342773
-0.23596981167793274
-0.2259826362133026
-0.21598957479000092
-0.20588037371635437
-0.19635246694087982
-0.1793651431798935
-0.17934225499629974
-0.16819153726100922
-0.5640231370925903
-0.7452517747879028
-0.732900857925415
-0.7360450029373169
-0.7342157959938049
-0.7375803589820862
-0.7362714409828186
-0.73682701587677
-0.7364663481712341
-0.7366650700569153
-0.7365705370903015
-0.7366182208061218
-0.7365930676460266
-0.7366061210632324
-0.7365995049476624
-0.7366030812263489
-0.7366015911102295
-0.7366019487380981
-0.7366012334823608
-0.7366016507148743
-0.7366024851799011
-0.7366016507148743
-0.7366018295288086
-0.7366015315055847
-0.736601710319519
-0.7366015911102295
-0.7366019487380981
-0.736602246761322
-0.7366021275520325
-0.736602246761322
-0.7366021871566772
-0.7366020679473877
-0.7366021275520325
-0.7366020679473877
-0.7366021275520325
-0.7366020083427429
-0.7366020679473877
-0.7366021275520325
-0.7366021871566772
-0.7366021871566772
-0.7366015911102295
-0.7366018295288086
-0.7366017699241638
-0.7366019487380981
-0.7366019487380981
-0.7366015315055847
-0.7366015315055847
-0.7366018295288086
-0.7366018891334534
-0.7366014122962952
-0.736601710319519
-0.7366017699241638
-0.7366018295288086
-0.7366017699241638
-0.736601710319519
-0.7366019487380981
-0.7366019487380981
-0.7366019487380981
-0.7366019487380981
-0.7366020679473877
-0.7366020679473877
-0.7366021871566772
-0.7366021871566772
-0.7366023063659668
-0.7366021871566772
-0.7366023659706116
-0.7366021275520325
-0.7366020679473877
-0.7366021871566772
-0.7366024255752563
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668
-0.7366023063659668

==> figs/2d_final_density/greenshields_godunov.tex <==
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152895450592041
0.5152717232704163
0.5152193307876587
0.5150850415229797
0.5147812962532043
0.5141794085502625
0.5131310224533081
0.5115020871162415
0.5091917514801025
0.5060657262802124
0.49086862802505493
0.4852542579174042
0.4800543785095215
0.47505873441696167
0.47019776701927185
0.46544039249420166
0.46077248454093933
0.45618680119514465
0.45168209075927734
0.44725990295410156
0.4429241120815277
0.4386807680130005
0.4345382750034332
0.43050646781921387
0.42659708857536316
0.4228237569332123
0.41920191049575806
0.41574805974960327
0.41248002648353577
0.4094163775444031
0.4065753221511841
0.40397387742996216
0.401626318693161
0.3995434641838074
0.3977300226688385
0.3961838483810425
0.3948942720890045
0.39384061098098755
0.39299044013023376
0.3922977149486542
0.3917014002799988
0.40910252928733826
0.703483521938324
0.8098188042640686
0.8138768076896667
0.8108487725257874
0.8073228597640991
0.8036710619926453
0.799924373626709
0.7960934638977051
0.7921864986419678
0.7882105112075806
0.7841716408729553
0.7800753116607666
0.7759260535240173
0.7717283964157104
0.7674860954284668
0.7632027268409729
0.7588819861412048
0.7545263767242432
0.7501389980316162
0.7457223534584045
0.7412789463996887
0.7368109226226807
0.7323208451271057
0.7278105020523071
0.723281979560852
0.7187370657920837
0.7141779065132141
0.7096061706542969
0.7050235867500305
0.7004322409629822
0.6958339810371399
0.6912309527397156
0.6866251826286316
0.6820192337036133
0.6774153709411621
0.6728166937828064
0.668226420879364
0.6636484265327454
0.6590871214866638
0.6545476317405701
0.6500362753868103
0.6455606818199158
0.6411297917366028
0.6367552876472473
0.6324512958526611
0.6282365918159485
0.6241360306739807
0.620185911655426
0.6164441704750061
0.6130156517028809
0.6101139783859253
0.6082085371017456
0.6083393692970276
0.6125787496566772
0.6238713264465332
0.6433655619621277
0.6667121052742004
0.6866356730461121
0.6994506120681763
0.705912172794342
0.7082101106643677
0.7081264853477478
0.7067352533340454
0.7046096920967102
0.7020419836044312
0.6991804838180542
0.69610196352005
0.6928491592407227
0.6894474029541016
0.6859143376350403
0.6822629570960999
0.6785041093826294
0.6746476888656616
0.6707015633583069
0.6666737794876099
0.6625714898109436
0.6584009528160095
0.6541680693626404
0.6498777866363525
0.645534873008728
0.6411435604095459
0.6367077231407166
0.6322306394577026
0.6277153491973877
0.623164713382721
0.6185809969902039
0.6139662861824036
0.6093227863311768
0.6046516299247742
0.5999545454978943
0.5952320694923401
0.5904855728149414
0.5857155919075012
0.5809224247932434
0.5761060118675232
0.5712662935256958
0.5664027333259583
0.561514139175415
0.5565989017486572
0.5516546964645386
0.5466777682304382
0.5416631698608398
0.5366029739379883
0.5314860939979553
0.5262911319732666
0.5209829807281494
0.5154852271080017
0.5095744132995605
0.4913768172264099
0.48612725734710693
0.4813188910484314
0.47676223516464233
0.4724022448062897
0.4682231843471527
0.464226633310318
0.4604240357875824
0.45683377981185913
0.4534773528575897
0.45038071274757385
0.44756948947906494
0.5229088664054871
0.6289688348770142
0.6368294358253479
0.6370688676834106
0.6370747089385986
0.6370757818222046
0.6370768547058105
0.6370779275894165
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672

==> figs/2d_final_density/greenshields_lax_hopf.tex <==
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152965784072876
0.5152958035469055
0.5126503109931946
0.5076403021812439
0.5026302337646484
0.49762025475502014
0.49261021614074707
0.4876002073287964
0.4825901687145233
0.47758015990257263
0.47257015109062195
0.4675601124763489
0.4625501036643982
0.4575400948524475
0.45253005623817444
0.44752004742622375
0.4425100088119507
0.4375
0.4324899911880493
0.42747995257377625
0.42246994376182556
0.4174599349498749
0.4124498963356018
0.4074398875236511
0.40242984890937805
0.39741984009742737
0.3924882411956787
0.3909395933151245
0.3909395933151245
0.3909395933151245
0.3909395933151245
0.3909395933151245
0.3909395933151245
0.3909395933151245
0.3909395933151245
0.3909395933151245
0.5261251330375671
0.8383015990257263
0.8332915902137756
0.828281581401825
0.8232715129852295
0.8182615041732788
0.8132514953613281
0.8082414865493774
0.8032314777374268
0.7982214689254761
0.7932114005088806
0.7882013916969299
0.7831913828849792
0.7781813740730286
0.7731713652610779
0.7681612968444824
0.7631512880325317
0.758141279220581
0.7531312704086304
0.7481212615966797
0.7431111931800842
0.7381011843681335
0.7330911755561829
0.7280811667442322
0.7230711579322815
0.7180611491203308
0.7130510807037354
0.7080410718917847
0.703031063079834
0.6980210542678833
0.6930110454559326
0.6880009770393372
0.6829909682273865
0.6779809594154358
0.6729709506034851
0.6679609417915344
0.662950873374939
0.6579408645629883
0.6529308557510376
0.6479208469390869
0.6429108381271362
0.6379008293151855
0.6328907608985901
0.6278807520866394
0.6228707432746887
0.617860734462738
0.6128507256507874
0.6078406572341919
0.6028306484222412
0.5978206396102905
0.5942883491516113
0.5941880345344543
0.5941880345344543
0.5941880345344543
0.5941880345344543
0.5941880345344543
0.5941880345344543
0.7196089029312134
0.7262099981307983
0.7262099981307983
0.7262099981307983
0.7262099981307983
0.7262099981307983
0.7261712551116943
0.7230711579322815
0.7180611491203308
0.7130510807037354
0.7080410718917847
0.703031063079834
0.6980210542678833
0.6930110454559326
0.6880009770393372
0.6829909682273865
0.6779809594154358
0.6729709506034851
0.6679609417915344
0.662950873374939
0.6579408645629883
0.6529308557510376
0.6479208469390869
0.6429108381271362
0.6379008293151855
0.6328907608985901
0.6278807520866394
0.6228707432746887
0.617860734462738
0.6128507256507874
0.6078406572341919
0.6028306484222412
0.5978206396102905
0.5928106307983398
0.5878006219863892
0.5827905535697937
0.577780544757843
0.5727705359458923
0.5677605271339417
0.562750518321991
0.5577405095100403
0.5527304410934448
0.5477204322814941
0.5427104234695435
0.5377004146575928
0.5326904058456421
0.5276803374290466
0.522670328617096
0.5176603198051453
0.5126503109931946
0.5076403021812439
0.5026302337646484
0.49762025475502014
0.49261021614074707
0.4876002073287964
0.4825901687145233
0.47758015990257263
0.47257015109062195
0.4675601124763489
0.4625501036643982
0.4575400948524475
0.45253005623817444
0.44752004742622375
0.4425100088119507
0.4878644645214081
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672
0.6370790600776672

==> figs/2d_final_density/greenshields_ours.tex <==
0.5152965784072876
0.5152966976165771
0.5152974724769592
0.515291154384613
0.5152859687805176
0.5153083801269531
0.5153279304504395
0.515264093875885
0.5151978135108948
0.5153522491455078
0.5156025290489197
0.515348494052887
0.5146461725234985
0.5149251222610474
0.5170273780822754
0.5189976096153259
0.5182276964187622
0.5145143270492554
0.5092819333076477
0.5037371516227722
0.4983249008655548
0.49306434392929077
0.48788028955459595
0.48271605372428894
0.4775465428829193
0.47236090898513794
0.46715664863586426
0.4619339108467102
0.4566972553730011
0.45144981145858765
0.44619491696357727
0.44093403220176697
0.43567121028900146
0.4304041564464569
0.42512989044189453
0.419872522354126
0.4147248864173889
0.40978458523750305
0.40478527545928955
0.39865586161613464
0.3904189169406891
0.38238954544067383
0.3814713656902313
0.3883776068687439
0.3932391107082367
0.392082542181015
0.3903523087501526
0.3914656341075897
0.38715454936027527
0.39588966965675354
0.38529717922210693
0.5817810297012329
0.8473901748657227
0.8292830586433411
0.8275765180587769
0.8205224871635437
0.8175119161605835
0.8115050196647644
0.8070197105407715
0.8018397092819214
0.7969868183135986
0.791981041431427
0.7870543599128723
0.7820949554443359
0.7771568298339844
0.7722150087356567
0.7672808170318604
0.762349009513855
0.7574217319488525
0.7524973154067993
0.7475767731666565
0.7426581382751465
0.7377426624298096
0.7328295707702637
0.727917492389679
0.723005473613739
0.7180938124656677
0.7131830453872681
0.7082730531692505
0.7033630013465881
0.6984503269195557
0.6935341358184814
0.6886156797409058
0.6836957335472107
0.6787719130516052
0.6738439202308655
0.6689122915267944
0.6639752388000488
0.6590309739112854
0.6540805697441101
0.6491237878799438
0.644158124923706
0.6391826272010803
0.6341962814331055
0.6291981339454651
0.6241852045059204
0.6191555857658386
0.6141045689582825
0.6090258359909058
0.6039115786552429
0.598787784576416
0.5939528942108154
0.5903622508049011
0.5892085433006287
0.5914104580879211
0.5939353108406067
0.5895769000053406
0.6173793077468872
0.7027609944343567
0.7303382158279419
0.7260082364082336
0.7260631918907166
0.7274481058120728
0.7267815470695496
0.7241143584251404
0.720902681350708
0.716841459274292
0.7124273180961609
0.7078233957290649
0.7031176090240479
0.6983321905136108
0.6934961080551147
0.6886268258094788
0.6837345957756042
0.6788235902786255
0.673900306224823
0.6689661741256714
0.6640234589576721
0.6590723991394043
0.6541143655776978
0.6491501927375793
0.644180178642273
0.6392041444778442
0.6342214941978455
0.6292337775230408
0.624239444732666
0.6192377805709839
0.6142292022705078
0.6092140674591064
0.6041923761367798
0.599162757396698
0.5941259264945984
0.5890824198722839
0.5840329527854919
0.5789779424667358
0.573915958404541
0.5688484907150269
0.5637750625610352
0.5586950182914734
0.5536081194877625
0.5485159158706665
0.5434171557426453
0.5383119583129883
0.5331985354423523
0.5280779600143433
0.5229493379592896
0.5178112387657166
0.5126634836196899
0.5075067281723022
0.502341091632843
0.4971671998500824
0.49198412895202637
0.4867894947528839
0.481587290763855
0.47637125849723816
0.47115761041641235
0.4659140706062317
0.4606579542160034
0.45567795634269714
0.44845959544181824
0.45273828506469727
0.43821975588798523
0.45899567008018494
0.6367613077163696
0.6387534141540527
0.6379777789115906
0.6360737681388855
0.6375612020492554
0.6369374990463257
0.6370980739593506
0.6370853185653687
0.6370751857757568
0.6370812654495239
0.6370795369148254
0.6370787024497986
0.6370794177055359
0.6370788812637329
0.6370801329612732
0.6370797157287598
0.6370785236358643
0.637080192565918
0.6370797753334045
0.6370787620544434
0.6370804905891418
0.6370803117752075
0.6370792388916016
0.6370800137519836
0.637079656124115
0.637079656124115
0.6370790600776672

==> figs/2d_final_density/triangular_godunov.tex <==
0.5
0.522359311580658
0.5170860290527344
0.5124228596687317
0.5085509419441223
0.5055426955223083
0.5033642053604126
0.5019003748893738
0.5009922981262207
0.5004753470420837
0.5002070665359497
0.5000813603401184
0.5000286102294922
0.5000091195106506
0.5000029802322388
0.5000014901161194
0.5000011920928955
0.5000008940696716
0.5000005960464478
0.5000002980232239
0.49999985098838806
0.4999997019767761
0.4999995529651642
0.49999919533729553
0.4999970495700836
0.49998727440834045
0.49995148181915283
0.4998399317264557
0.4995376467704773
0.498814195394516
0.4972652494907379
0.49426791071891785
0.48898279666900635
0.4804314374923706
0.46765968203544617
0.44996175169944763
0.4271068274974823
0.3994935154914856
0.3681723177433014
0.33471614122390747
0.3009694218635559
0.26874515414237976
0.23955009877681732
0.21440239250659943
0.19377006590366364
0.17762167751789093
0.16555482149124146
0.15695945918560028
0.15117976069450378
0.14764992892742157
0.14599139988422394
0.14606407284736633
0.14796452224254608
0.15196819603443146
0.6329306960105896
0.832298994064331
0.8103061318397522
0.7833358645439148
0.751939058303833
0.7171923518180847
0.6807041168212891
0.6444272398948669
0.6103649139404297
0.5802430510520935
0.5552323460578918
0.5358008742332458
0.5217296481132507
0.5122743844985962
0.5064087510108948
0.5030691027641296
0.5013361573219299
0.5005232095718384
0.500182032585144
0.5000554919242859
0.5000147223472595
0.5000036954879761
0.5000012516975403
0.5000008940696716
0.5000005960464478
0.5000002980232239
0.49999985098838806
0.4999997019767761
0.4999995529651642
0.49999916553497314
0.4999966621398926
0.49998533725738525
0.4999437928199768
0.49981430172920227
0.4994634687900543
0.49862390756607056
0.49682629108428955
0.4933478832244873
0.48721450567245483
0.4772907793521881
0.46246930956840515
0.4419310688972473
0.4154081344604492
0.38336315751075745
0.3470152020454407
0.3081895411014557
0.2690267562866211
0.23163074254989624
0.19775012135505676
0.1685665100812912
0.14462335407733917
0.12588536739349365
0.11188939958810806
0.10193801671266556
0.09529423713684082
0.09134983271360397
0.0897504910826683
0.09046439826488495
0.09377995133399963
0.1002223864197731
0.45995795726776123
0.7882918119430542
0.7691566944122314
0.7457603216171265
0.71852707862854
0.688388466835022
0.656739354133606
0.6252734065055847
0.5957285761833191
0.5696013569831848
0.5479074716567993
0.5310528874397278
0.5188477635383606
0.510646402835846
0.5055585503578186
0.5026618838310242
0.5011587738990784
0.5004538297653198
0.5001579523086548
0.5000482201576233
0.500012993812561
0.5000033378601074
0.5000011920928955
0.5000008940696716
0.5000005960464478
0.5000002980232239
0.49999985098838806
0.4999997019767761
0.4999995529651642
0.4999992847442627
0.4999975860118866
0.4999898374080658
0.499961256980896
0.49987220764160156
0.49963104724884033
0.49905380606651306
0.4978179335594177
0.4954265058040619
0.4912097752094269
0.48438704013824463
0.4741970896720886
0.4600767195224762
0.44184184074401855
0.4198104739189148
0.3948206901550293
0.3681275248527527
0.3412024676799774
0.3154921531677246
0.29219868779182434
0.272134393453598
0.2556723952293396
0.2427864521741867
0.23315201699733734
0.22627294063568115
0.22160401940345764
0.2186499387025833
0.21703168749809265
0.2165188491344452
0.2170286327600479
0.21859443187713623
0.22130979597568512
0.22525833547115326
0.2304464429616928
0.23675602674484253
0.24393151700496674
0.2516043186187744
0.25934723019599915
0.26674219965934753
0.2734425961971283
0.2792142927646637
0.28394943475723267
0.2876543402671814
0.2904185950756073
0.29237478971481323
0.29365628957748413
0.2943587303161621
0.2945087254047394
0.2940457761287689
0.2928226590156555
0.29063063859939575
0.2872483432292938
0.2825080454349518
0.2763609290122986
0.2689220905303955
0.2604789137840271
0.29603469371795654

==> figs/2d_final_density/triangular_lax_hopf.tex <==
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.15906085073947906
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.1411166787147522
0.738914430141449
0.8883638978004456
0.8883638978004456
0.8883638978004456
0.8883638978004456
0.8883638978004456
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.1043429747223854
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.08351892232894897
0.6108570694923401
0.8368591666221619
0.8368591666221619
0.8368591666221619
0.8368591666221619
0.8368591666221619
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.22798000276088715
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.21366316080093384
0.2919161319732666
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654
0.29603469371795654

==> figs/2d_final_density/triangular_ours.tex <==
0.5
0.5113641023635864
0.5022833347320557
0.5101271867752075
0.5040627121925354
0.5070278644561768
0.5042788982391357
0.5049487948417664
0.5036898255348206
0.5034834742546082
0.50278639793396
0.5023424029350281
0.501835823059082
0.5013880133628845
0.500953197479248
0.5005698204040527
0.5001732110977173
0.49986496567726135
0.49948930740356445
0.49924784898757935
0.4988722503185272
0.49869024753570557
0.4982920289039612
0.49817749857902527
0.49773532152175903
0.497721791267395
0.4972083866596222
0.49735960364341736
0.4967220723628998
0.497140496969223
0.4962693154811859
0.4971183240413666
0.49579930305480957
0.49735352396965027
0.4952073395252228
0.4979556202888489
0.49419066309928894
0.49788734316825867
0.4907165467739105
0.46160468459129333
0.21230469644069672
0.13332849740982056
0.1475348174571991
0.12501974403858185
0.14267536997795105
0.1400136649608612
0.14100448787212372
0.14154323935508728
0.14093109965324402
0.14119952917099
0.1411077380180359
0.14063841104507446
0.1439966857433319
0.16070343554019928
0.761997640132904
0.8879415988922119
0.9003663063049316
0.8761740922927856
0.9117426872253418
0.8562098741531372
0.567302405834198
0.5044574737548828
0.5034917593002319
0.5003978610038757
0.5015855431556702
0.5001750588417053
0.5013866424560547
0.5003629326820374
0.5013075470924377
0.5007100701332092
0.5015465617179871
0.5013630390167236
0.5020125508308411
0.5018738508224487
0.502030074596405
0.501700758934021
0.5014505386352539
0.5010404586791992
0.5006090402603149
0.5002275109291077
0.49973759055137634
0.49943530559539795
0.49893102049827576
0.4987374544143677
0.49822038412094116
0.49816378951072693
0.4976043105125427
0.497724711894989
0.49706050753593445
0.4974285960197449
0.49655407667160034
0.4972977638244629
0.49603337049484253
0.49737927317619324
0.495415598154068
0.4977594017982483
0.4943222999572754
0.4973113238811493
0.49202242493629456
0.446579247713089
0.14229212701320648
0.06915390491485596
0.09167997539043427
0.06777475774288177
0.08556247502565384
0.0827791690826416
0.08321964740753174
0.08398056030273438
0.08336856961250305
0.08348025381565094
0.08364859223365784
0.08305114507675171
0.08601371943950653
0.08034256845712662
0.5834107398986816
0.8414794206619263
0.8429118990898132
0.8234591484069824
0.8590906262397766
0.803346574306488
0.5550243854522705
0.5049312710762024
0.5033966302871704
0.5010456442832947
0.5022042393684387
0.5008838176727295
0.5021359920501709
0.5010963082313538
0.5021187663078308
0.5014953017234802
0.5023751258850098
0.5021238327026367
0.5027034282684326
0.5024629235267639
0.5025361776351929
0.5021735429763794
0.5018995404243469
0.5015249252319336
0.5011094808578491
0.5008071064949036
0.500353217124939
0.5001645684242249
0.4997067451477051
0.4996594190597534
0.49919217824935913
0.49931102991104126
0.49879932403564453
0.4991121292114258
0.49849647283554077
0.49904072284698486
0.49824604392051697
0.4990725517272949
0.49802133440971375
0.4991859495639801
0.49782252311706543
0.49932917952537537
0.49747052788734436
0.4982888996601105
0.4951639175415039
0.4442940950393677
0.22244618833065033
0.2110167145729065
0.21785669028759003
0.20105530321598053
0.21772883832454681
0.2119034081697464
0.214072585105896
0.21388310194015503
0.21342667937278748
0.21386000514030457
0.21349717676639557
0.2138536423444748
0.21338580548763275
0.21406827867031097
0.21288663148880005
0.21443435549736023
0.21313214302062988
0.21467354893684387
0.21742142736911774
0.23500606417655945
0.28095221519470215
0.30298155546188354
0.29670262336730957
0.29827404022216797
0.2965310215950012
0.2956608235836029
0.29630225896835327
0.2958417534828186
0.29614776372909546
0.2958952784538269
0.29627472162246704
0.295585572719574
0.2966839075088501
0.294916570186615
0.29765912890434265
0.29567983746528625
0.30020055174827576
0.2990620732307434
0.2868608236312866
0.29603469371795654

==> figs/lwr_example/2D.tex <==
0.5
0.4998083710670471
0.49937957525253296
0.5005395412445068
0.5005177855491638
0.5016687512397766
0.5012894868850708
0.5019314289093018
0.501660943031311
0.5020740032196045
0.5019692182540894
0.502142071723938
0.5020089745521545
0.5019432306289673
0.5017165541648865
0.5014913082122803
0.5012151002883911
0.5009199380874634
0.5006445646286011
0.5003355741500854
0.5000935196876526
0.4997985064983368
0.49961012601852417
0.499339759349823
0.4992187023162842
0.49897199869155884
0.49892738461494446
0.49869319796562195
0.49873197078704834
0.498491108417511
0.4986186623573303
0.4983483850955963
0.498569518327713
0.49825140833854675
0.4985654652118683
0.4981963336467743
0.4985795021057129
0.49819204211235046
0.49856123328208923
0.49828019738197327
0.49836716055870056
0.4981608986854553
0.4965137541294098
0.4966209828853607
0.4219251275062561
0.20376962423324585
0.21242304146289825
0.20561343431472778
0.19326737523078918
0.2108510434627533
0.2039085328578949
0.2069631665945053
0.20642569661140442
0.20600222051143646
0.20641069114208221
0.2061917930841446
0.20619970560073853
0.20633195340633392
0.20611609518527985
0.20630677044391632
0.2064618319272995
0.20590472221374512
0.2070070058107376
0.207499161362648
0.21358132362365723
0.21052126586437225
0.20467275381088257
0.2035626918077469
0.20602692663669586
0.20431479811668396
0.20703203976154327
0.19504570960998535
0.26143959164619446
0.4392188489437103
0.4930245280265808
0.4965536892414093
0.500144362449646
0.49949583411216736
0.4996420741081238
0.49930307269096375
0.49911412596702576
0.49882274866104126
0.49859583377838135
0.4982966184616089
0.49808403849601746
0.49777957797050476
0.4976065456867218
0.49729838967323303
0.4971940219402313
0.4968651235103607
0.49687397480010986
0.49648621678352356
0.49666598439216614
0.4961765706539154
0.49658551812171936
0.49599674344062805
0.49671804904937744
0.49599605798721313
0.4970167875289917
0.4956149756908417
0.49721869826316833
0.4940713346004486
0.496891587972641
0.4859652817249298
0.4481063485145569
0.19969896972179413
0.13780276477336884
0.08159533143043518
0.5047101974487305
0.5404290556907654
0.5654637813568115
0.5602045655250549
0.5467360019683838
0.568868100643158
0.5412762761116028
0.5066947340965271
0.5139741897583008
0.5032105445861816
0.51027911901474
0.5047752857208252
0.5075654983520508
0.5052531957626343
0.5056985020637512
0.5048666000366211
0.5044178366661072
0.5040645599365234
0.5034164190292358
0.5031434893608093
0.5025335550308228
0.5022374391555786
0.5017145872116089
0.5013939142227173
0.5009523034095764
0.5006276965141296
0.5002539753913879
0.49994251132011414
0.49962523579597473
0.4993351697921753
0.49906373023986816
0.49879348278045654
0.49855515360832214
0.49829602241516113
0.4980778694152832
0.49781927466392517
0.49761298298835754
0.4973489046096802
0.4971543252468109
0.4968852400779724
0.49671003222465515
0.49644070863723755
0.4962983727455139
0.4960349202156067
0.4959416389465332
0.49568694829940796
0.4956614673137665
0.49540975689888
0.4954744577407837
0.4951997697353363
0.49538376927375793
0.4950282871723175
0.49535056948661804
0.49420323967933655
0.49366360902786255
0.4939954876899719
0.395256906747818
0.06246895343065262
0.025522476062178612
0.018795782700181007
0.002705177990719676
0.01089773140847683
0.006216844543814659
0.007339731324464083
0.0027436756063252687
0.007683330215513706
0.004047734662890434
0.03517869487404823
0.014835653826594353
0.20933358371257782
0.43954241275787354
0.48682087659835815
0.4961320459842682
0.498515784740448
0.4982924163341522
0.4982451796531677
0.49795496463775635
0.4976981580257416
0.49747928977012634
0.4971778392791748
0.4971564710140228
0.4965599775314331
0.4971054792404175
0.49650827050209045
0.49665385484695435
0.49847865104675293
0.5000186562538147
0.5023900866508484
0.5008964538574219
0.5011034607887268
0.5000091791152954
0.5

==> figs/lwr_example/exact.tex <==
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.4853120744228363
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.22085866332054138
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.39668887853622437
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.4803692400455475
0.1073845624923706
0.1073845624923706
0.1073845624923706
0.56078040599823
0.56078040599823
0.56078040599823
0.56078040599823
0.56078040599823
0.56078040599823
0.56078040599823
0.5060780644416809
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.4753919541835785
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.03244730085134506
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5
0.5

==> figs/lwr_example/godunov.tex <==
0.5
0.5259836912155151
0.5165452361106873
0.5099675059318542
0.505657970905304
0.5030126571655273
0.5014974474906921
0.5006910562515259
0.5002944469451904
0.500115156173706
0.5000412464141846
0.5000138282775879
0.500004768371582
0.5000022649765015
0.5000017881393433
0.5000014901161194
0.5000011920928955
0.5000008940696716
0.5000005960464478
0.5000002980232239
0.49999985098838806
0.4999997019767761
0.4999995529651642
0.49999940395355225
0.4999992549419403
0.49999910593032837
0.4999985992908478
0.49999627470970154
0.4999881088733673
0.49996328353881836
0.4998966157436371
0.4997343122959137
0.4993739128112793
0.49863889813423157
0.4972534477710724
0.49482715129852295
0.49086254835128784
0.48479360342025757
0.47606056928634644
0.46421101689338684
0.44900819659233093
0.4305192232131958
0.409156858921051
0.38565900921821594
0.3610062301158905
0.33629393577575684
0.3125879168510437
0.29079383611679077
0.2715655267238617
0.25526493787765503
0.24197213351726532
0.23153461515903473
0.22363771498203278
0.21787910163402557
0.213833749294281
0.21110139787197113
0.2093346267938614
0.20824992656707764
0.2076263278722763
0.20729731023311615
0.207140251994133
0.2070668339729309
0.2070157676935196
0.20694835484027863
0.20685425400733948
0.20680560171604156
0.20714972913265228
0.20890189707279205
0.21414780616760254
0.2259245216846466
0.2471325844526291
0.27880167961120605
0.31885796785354614
0.36244580149650574
0.40374964475631714
0.4381695091724396
0.4635990560054779
0.48036932945251465
0.4902985692024231
0.49560266733169556
0.4981699585914612
0.49929994344711304
0.49975359439849854
0.4999200999736786
0.49997594952583313
0.4999929368495941
0.4999968707561493
0.4999948740005493
0.49998417496681213
0.4999511241912842
0.4998619854450226
0.49964502453804016
0.49916335940361023
0.49818098545074463
0.4963292181491852
0.49308648705482483
0.4877876937389374
0.47967639565467834
0.4680044651031494
0.45216718316078186
0.4318482279777527
0.4071374535560608
0.3786053955554962
0.3475496172904968
0.3173888027667999
0.2976302206516266
0.31074297428131104
0.4062024652957916
0.5512426495552063
0.5535969734191895
0.5508225560188293
0.547460675239563
0.5435042381286621
0.5390164256095886
0.5341261029243469
0.529017448425293
0.5239095687866211
0.5190297961235046
0.5145826935768127
0.5107242465019226
0.5075434446334839
0.505057692527771
0.5032206773757935
0.5019404888153076
0.5011017322540283
0.5005870461463928
0.5002921223640442
0.5001351833343506
0.500058114528656
0.5000234246253967
0.5000091791152954
0.5000039339065552
0.500002384185791
0.5000020861625671
0.5000017881393433
0.5000014901161194
0.5000011920928955
0.5000008940696716
0.5000005960464478
0.5000002980232239
0.49999985098838806
0.4999997019767761
0.4999995529651642
0.49999940395355225
0.4999992549419403
0.49999910593032837
0.49999815225601196
0.4999941289424896
0.4999803900718689
0.49993884563446045
0.4998270869255066
0.4995551109313965
0.4989513158798218
0.4977199137210846
0.495398610830307
0.4913336932659149
0.4846913516521454
0.47452354431152344
0.45989227294921875
0.4400395452976227
0.41456884145736694
0.3835926353931427
0.3478023111820221
0.30843424797058105
0.2671312987804413
0.22572991251945496
0.18602178990840912
0.14955386519432068
0.11753479391336441
0.09091587364673615
0.07067160308361053
0.058188583701848984
0.05550409480929375
0.06506527215242386
0.08886861056089401
0.12726347148418427
0.17806394398212433
0.23657459020614624
0.29665330052375793
0.3523423373699188
0.39931759238243103
0.4355897009372711
0.4613477289676666
0.47823646664619446
0.4884953200817108
0.49428555369377136
0.4973296821117401
0.4988216161727905
0.4994971752166748
0.4997580349445343
0.4997827708721161
0.4995969533920288
0.4990994930267334
0.4980570673942566
0.4960833787918091
0.4926246106624603
0.48697203397750854
0.47831904888153076
0.4658675491809845
0.5

==> figs/lwr_example/ic.tex <==
0.8122923374176025
0.8122923374176025
0.8122923374176025
0.8122923374176025
0.8122923374176025
0.8122923374176025
0.8122923374176025
0.8122923374176025
0.8122923374176025
0.8122923374176025
0.8122923374176025
0.8122923374176025
0.8122923374176025
0.8122923374176025
0.8122923374176025
0.8122923374176025
0.8122923374176025
0.8122923374176025
0.8122923374176025
0.8122923374176025
0.22092947363853455
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.20624154806137085
0.21958407759666443
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.20482534170150757
0.6478613018989563
0.6711789965629578
0.6711789965629578
0.6711789965629578
0.6711789965629578
0.6711789965629578
0.6711789965629578
0.6711789965629578
0.6711789965629578
0.6711789965629578
0.6711789965629578
0.6711789965629578
0.6711789965629578
0.6711789965629578
0.6711789965629578
0.6711789965629578
0.6711789965629578
0.6711789965629578
0.6711789965629578
0.6711789965629578
0.12701533734798431
0.1073845624923706
0.1073845624923706
0.1073845624923706
0.1073845624923706
0.1073845624923706
0.1073845624923706
0.1073845624923706
0.1073845624923706
0.1073845624923706
0.1073845624923706
0.1073845624923706
0.1073845624923706
0.1073845624923706
0.1073845624923706
0.1073845624923706
0.1073845624923706
0.1073845624923706
0.1073845624923706
0.1073845624923706
0.7585607171058655
0.792833149433136
0.792833149433136
0.792833149433136
0.792833149433136
0.792833149433136
0.792833149433136
0.792833149433136
0.792833149433136
0.792833149433136
0.792833149433136
0.792833149433136
0.792833149433136
0.792833149433136
0.792833149433136
0.792833149433136
0.792833149433136
0.792833149433136
0.792833149433136
0.792833149433136
0.5577414035797119
0.56078040599823
0.56078040599823
0.56078040599823
0.56078040599823
0.56078040599823
0.56078040599823
0.56078040599823
0.56078040599823
0.56078040599823
0.56078040599823
0.56078040599823
0.56078040599823
0.56078040599823
0.56078040599823
0.56078040599823
0.56078040599823
0.56078040599823
0.56078040599823
0.56078040599823
0.03244730085134506
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.00783926248550415
0.6387109160423279
0.6719146966934204
0.6719146966934204
0.6719146966934204
0.6719146966934204
0.6719146966934204
0.6719146966934204
0.6719146966934204
0.6719146966934204
0.6719146966934204
0.6719146966934204
0.6719146966934204
0.6719146966934204
0.6719146966934204
0.6719146966934204
0.6719146966934204
0.6719146966934204
0.6719146966934204
0.6719146966934204
0.6719146966934204
0.10210432857275009
0.0811624526977539
0.0811624526977539
0.0811624526977539
0.0811624526977539
0.0811624526977539
0.0811624526977539
0.0811624526977539
0.0811624526977539
0.0811624526977539
0.0811624526977539
0.0811624526977539
0.0811624526977539
0.0811624526977539
0.0811624526977539
0.0811624526977539
0.0811624526977539
0.0811624526977539
0.0811624526977539
0.0811624526977539

==> figs/lwr_example/unsupervised.tex <==
0.5
0.5243052244186401
0.5118957757949829
0.508588969707489
0.5050740242004395
0.5027307868003845
0.5012794733047485
0.5005035400390625
0.5001515746116638
0.5000045895576477
0.49987298250198364
0.4997391998767853
0.49960750341415405
0.49948108196258545
0.49936309456825256
0.49925628304481506
0.4991621673107147
0.49908098578453064
0.4990116357803345
0.4989525377750397
0.4989018440246582
0.4988579750061035
0.4988197684288025
0.4987860918045044
0.49875620007514954
0.49872922897338867
0.49870479106903076
0.49868232011795044
0.4986617863178253
0.4986429810523987
0.49862557649612427
0.49860939383506775
0.49859383702278137
0.4985796809196472
0.49856865406036377
0.4985421299934387
0.49852344393730164
0.49893733859062195
0.49397140741348267
0.4804724156856537
0.4671499729156494
0.449122816324234
0.4263160228729248
0.39968252182006836
0.3707452416419983
0.3413357734680176
0.31324705481529236
0.2879353165626526
0.26634088158607483
0.24884691834449768
0.23535440862178802
0.22542381286621094
0.21843424439430237
0.2137216031551361
0.2106761336326599
0.20879551768302917
0.20770007371902466
0.20712126791477203
0.20687681436538696
0.20683839917182922
0.2069123536348343
0.2070353627204895
0.20712663233280182
0.20710454881191254
0.20708192884922028
0.2071962207555771
0.206862211227417
0.20508943498134613
0.20311370491981506
0.20669934153556824
0.2239827811717987
0.2594313621520996
0.30954521894454956
0.364480197429657
0.4137347936630249
0.45096278190612793
0.47517555952072144
0.4902547001838684
0.49842891097068787
0.4990316331386566
0.49898067116737366
0.4989345669746399
0.49889424443244934
0.49885857105255127
0.4988264739513397
0.49879732728004456
0.49877044558525085
0.49874570965766907
0.49872294068336487
0.4987022280693054
0.4986831247806549
0.4986654818058014
0.498649001121521
0.49863171577453613
0.49861326813697815
0.49865201115608215
0.4985351860523224
0.4975183606147766
0.48468688130378723
0.4709470868110657
0.45198026299476624
0.42618221044540405
0.3950764834880829
0.3596879243850708
0.3161231279373169
0.26573121547698975
0.24676407873630524
0.36575502157211304
0.5551618337631226
0.5556644797325134
0.5536869764328003
0.5507922172546387
0.5472069978713989
0.5429610013961792
0.5381776094436646
0.5330653786659241
0.5279011726379395
0.5229925513267517
0.5186276435852051
0.5150234699249268
0.5121356844902039
0.509421169757843
0.5068615078926086
0.5046521425247192
0.5029160976409912
0.5016783475875854
0.5008814334869385
0.500420868396759
0.5001837015151978
0.5000738501548767
0.4999810457229614
0.4998761713504791
0.49976348876953125
0.4996477961540222
0.49953383207321167
0.49942639470100403
0.49932852387428284
0.49924182891845703
0.4991662800312042
0.4991008937358856
0.49904438853263855
0.4989950656890869
0.49895164370536804
0.49891290068626404
0.49887803196907043
0.49884647130966187
0.4988178312778473
0.4987918734550476
0.4987683892250061
0.49874719977378845
0.4987277388572693
0.4987093508243561
0.4986920654773712
0.4986790418624878
0.4986484944820404
0.4986107051372528
0.4991092085838318
0.49297744035720825
0.47847533226013184
0.46172964572906494
0.437091588973999
0.4040980339050293
0.36349695920944214
0.31723031401634216
0.2680906057357788
0.21918296813964844
0.17336079478263855
0.13281124830245972
0.0988263189792633
0.07163895666599274
0.05052904784679413
0.034843411296606064
0.025899602100253105
0.028163636103272438
0.04780818894505501
0.08888020366430283
0.14978371560573578
0.2228349894285202
0.2972046434879303
0.36311647295951843
0.4147822856903076
0.4509662687778473
0.47376900911331177
0.4875396490097046
0.496785044670105
0.49880093336105347
0.49878641963005066
0.49876126646995544
0.4987380802631378
0.4987173080444336
0.49869945645332336
0.4986853301525116
0.4986739456653595
0.4986504018306732
0.4985387623310089
0.4982600212097168
0.4981558918952942
0.5001463890075684
0.47354960441589355
0.5

==> figs/lwr_winrates/old_100ic/greenberg.tex <==
\def\mydata{
{-, 100, 100, 100, 100, 100, 100, 8},
{0, -, 71, 100, 72, 94, 95, 5},
{0, 29, -, 100, 33, 99, 99, 5},
{0, 0, 0, -, 0, 0, 1, 3},
{0, 28, 64, 100, -, 99, 99, 5},
{0, 6, 1, 100, 1, -, 100, 5},
{0, 5, 1, 99, 1, 0, -, 5},
{92, 95, 95, 97, 95, 95, 95, -},
}

==> figs/lwr_winrates/old_100ic/greenshield.tex <==
\def\mydata{
{-, 100, 100, 100, 100, 96, 96, 0},
{0, -, 100, 100, 100, 90, 90, 0},
{0, 0, -, 100, 59, 70, 70, 0},
{0, 0, 0, -, 0, 0, 0, 0},
{0, 0, 38, 100, -, 70, 70, 0},
{4, 10, 30, 100, 30, -, 92, 0},
{4, 10, 30, 100, 30, 8, -, 0},
{100, 100, 100, 100, 100, 100, 100, -},
}

==> figs/lwr_winrates/old_100ic/trapezoidal.tex <==
\def\mydata{
{-, 91, 99, 100, 100, 0, 0, 0},
{9, -, 100, 100, 100, 0, 0, 0},
{1, 0, -, 100, 83, 0, 0, 0},
{0, 0, 0, -, 0, 0, 0, 0},
{0, 0, 13, 100, -, 0, 0, 0},
{100, 100, 100, 100, 100, -, 0, 0},
{100, 100, 100, 100, 100, 100, -, 0},
{100, 100, 100, 100, 100, 100, 100, -},
}

==> figs/lwr_winrates/old_100ic/triangular.tex <==
\def\mydata{
{-, 100, 100, 100, 100, 63, 60, 0},
{0, -, 100, 100, 100, 47, 47, 0},
{0, 0, -, 100, 88, 43, 43, 0},
{0, 0, 0, -, 0, 0, 0, 0},
{0, 0, 9, 100, -, 43, 42, 0},
{37, 53, 57, 100, 57, -, 32, 0},
{40, 53, 57, 100, 58, 68, -, 1},
{100, 100, 100, 100, 100, 100, 99, -},
}

==> figs/lwr_winrates/old_100ic/triangular_skewed.tex <==
\def\mydata{
{-, 99, 99, 100, 99, 98, 98, 0},
{1, -, 93, 100, 93, 95, 95, 0},
{1, 7, -, 100, 78, 97, 97, 0},
{0, 0, 0, -, 0, 0, 0, 0},
{1, 7, 20, 100, -, 97, 97, 0},
{2, 5, 3, 100, 3, -, 99, 0},
{2, 5, 3, 100, 3, 1, -, 0},
{100, 100, 100, 100, 100, 100, 100, -},
}

==> figs/lwr_winrates/old_100ic/underwood.tex <==
\def\mydata{
{-, 100, 100, 100, 100, 0, 0, 0},
{0, -, 100, 100, 100, 0, 0, 0},
{0, 0, -, 100, 1, 0, 0, 0},
{0, 0, 0, -, 0, 0, 0, 0},
{0, 0, 4, 100, -, 0, 0, 0},
{100, 100, 100, 100, 100, -, 0, 0},
{100, 100, 100, 100, 100, 100, -, 1},
{100, 100, 100, 100, 100, 100, 99, -},
}

==> figs/lwr_winrates/winrates_greenberg.tex <==
\def\mydata{
{-, 98, 99, 100, 99, 100, 100, 6},
{2, -, 74, 100, 73, 96, 96, 3},
{1, 26, -, 100, 38, 98, 99, 3},
{0, 0, 0, -, 0, 0, 1, 2},
{1, 27, 60, 100, -, 99, 99, 3},
{0, 4, 2, 100, 1, -, 99, 3},
{0, 4, 2, 99, 1, 1, -, 3},
{94, 97, 97, 98, 97, 97, 97, -},
}

==> figs/lwr_winrates/winrates_greenshield.tex <==
\def\mydata{
{-, 99, 100, 100, 100, 96, 96, 0},
{1, -, 99, 100, 99, 90, 90, 0},
{0, 1, -, 100, 59, 71, 71, 0},
{0, 0, 0, -, 0, 0, 0, 0},
{0, 1, 40, 100, -, 71, 71, 0},
{4, 10, 30, 100, 30, -, 93, 0},
{4, 10, 29, 100, 29, 7, -, 0},
{100, 100, 100, 100, 100, 100, 100, -},
}

==> figs/lwr_winrates/winrates_trapezoidal.tex <==
\def\mydata{
{-, 94, 99, 100, 99, 0, 0, 0},
{6, -, 100, 100, 100, 0, 0, 0},
{1, 0, -, 100, 82, 0, 0, 0},
{0, 0, 0, -, 0, 0, 0, 0},
{1, 0, 3, 100, -, 0, 0, 0},
{100, 100, 100, 100, 100, -, 0, 0},
{100, 100, 100, 100, 100, 100, -, 0},
{100, 100, 100, 100, 100, 100, 100, -},
}

==> figs/lwr_winrates/winrates_triangular.tex <==
\def\mydata{
{-, 100, 100, 100, 100, 64, 63, 0},
{0, -, 100, 100, 100, 53, 52, 0},
{0, 0, -, 100, 87, 46, 46, 0},
{0, 0, 0, -, 0, 0, 0, 0},
{0, 0, 12, 100, -, 46, 45, 0},
{36, 47, 54, 100, 54, -, 32, 0},
{37, 48, 54, 100, 55, 68, -, 1},
{100, 100, 100, 100, 100, 100, 99, -},
}

==> figs/lwr_winrates/winrates_triangular_skewed.tex <==
\def\mydata{
{-, 99, 100, 100, 100, 98, 98, 0},
{1, -, 93, 100, 93, 96, 96, 0},
{0, 7, -, 100, 82, 97, 97, 0},
{0, 0, 0, -, 0, 0, 0, 0},
{0, 7, 16, 100, -, 97, 97, 0},
{2, 4, 3, 100, 3, -, 97, 0},
{2, 4, 3, 100, 3, 3, -, 0},
{100, 100, 100, 100, 100, 100, 100, -},
}

==> figs/lwr_winrates/winrates_underwood.tex <==
\def\mydata{
{-, 100, 100, 100, 100, 0, 0, 0},
{0, -, 100, 100, 100, 0, 0, 0},
{0, 0, -, 100, 2, 0, 0, 0},
{0, 0, 0, -, 0, 0, 0, 0},
{0, 0, 3, 100, -, 0, 0, 0},
{100, 100, 100, 100, 100, -, 0, 0},
{100, 100, 100, 100, 100, 100, -, 0},
{100, 100, 100, 100, 100, 100, 100, -},
}

==> header.tex <==
% Optional PDF information
\ifpdf
\hypersetup{
  pdftitle={Supervised and Unsupervised Neural Network Solver for First Order Hyperbolic Nonlinear PDEs},
  pdfauthor={D. Doe, P. T. Frank, and J. E. Smith}
}
\fi

% % Sets running headers as well as PDF title and authors
% \headers{An Example Article}{D. Doe, P. T. Frank, and J. E. Smith}

% % Title
% \title{On Supervised vs. Unsupervised Learning for First Order Hyperbolic Nonlinear PDEs\thanks{Submitted to the editors DATE.
% \funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}}

% % Authors: full names plus addresses.
% \author{Dianne Doe\thanks{Imagination Corp., Chicago, IL 
%   (\email{ddoe@imag.com}, \url{http://www.imag.com/\string~ddoe/}).}
% \and Paul T. Frank\thanks{Department of Applied Mathematics, Fictional University, Boise, ID 
%   (\email{ptfrank@fictional.edu}, \email{jesmith@fictional.edu}).}
% \and Jane E. Smith\footnotemark[3]}

% \usepackage{amsopn}
% \DeclareMathOperator{\diag}{diag}


% Sets running headers as well as PDF title and authors
\headers{An Example Article}{D. Doe, P. T. Frank, and J. E. Smith}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Supervised and Unsupervised Neural Network Solver for First Order Hyperbolic Nonlinear PDEs\thanks{Submitted to the editors DATE.
\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}}

% Authors: full names plus addresses.
\author{Dianne Doe\thanks{Imagination Corp., Chicago, IL 
  (\email{ddoe@imag.com}, \url{http://www.imag.com/\string~ddoe/}).}
\and Paul T. Frank\thanks{Department of Applied Mathematics, Fictional University, Boise, ID 
  (\email{ptfrank@fictional.edu}, \email{jesmith@fictional.edu}).}
\and Jane E. Smith\footnotemark[3]}



\DeclareMathOperator{\dt}{d\!}
\DeclareMathOperator{\riemann}{riemann}
\DeclareMathOperator{\Exp}{Exp}
\definecolor{darkmagenta}{rgb}{.38,0,0.38}
\usepackage{tikzscale}
\usepackage{amssymb}
% \usepackage{amsmath, amsthm}
\usepackage{adjustbox}
\usepackage{tabularx}
\renewcommand\tabularxcolumn[1]{m{#1}}
\def\tabularxcolumn#1{m{#1}}
\usepackage{afterpage}
\usepackage{adjustbox} 
\usepackage{dsfont}
\usepackage{placeins}
\usepackage{cleveref}
% \usepackage[table,xcdraw]{xcolor}  % already loaded in siamart250211.cls (\RequirePackage{xcolor}[2.11])
\usepackage{multirow}
\usepackage{makecell}
\usepackage{stackengine}
\usepackage{tikz}
\usepackage{float}
\usepackage{pgfplots}
\usepackage{mathtools}
\usepackage{lscape}
\usepackage{calc}
% \usepackage[T1]{fontenc}
% \usepackage[ansinew]{inputenc}
% \pdfmapfile{=ptm.map}
\usetikzlibrary{positioning, matrix, shapes.geometric, arrows.meta, fit, backgrounds, calc, intersections, fillbetween}
\usepgfplotslibrary{fillbetween}
\pgfplotsset{compat=1.18}
\usetikzlibrary{external}
% \tikzexternalize[prefix=tikz_figures/]
% \usepackage{subfigure}
\usepackage{tabu}
\usepackage{makecell}
\usepackage{array}
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcommand{\sizestd}{6}
\newcommand{\sizestdinter}{7}
\newcommand{\std}[1]{\color{black!70!white}\fontsize{\sizestd}{\sizestdinter}\selectfont ±#1}

\newcommand{\sizestdtiny}{4}
\newcommand{\sizestdintertiny}{5}
\newcommand{\tinystd}[1]{\color{black!70!white}\fontsize{\sizestdtiny}{\sizestdintertiny}\selectfont ±#1}

\usepackage{stmaryrd} % Required for \llbracket and \rrbracket
\newcommand{\inte}[2]{\llbracket #1, #2 \rrbracket}

\newcommand{\missingref}{\textcolor{red}{\textbf{[REF]}}}
\newcommand{\todo}{\textcolor{red}{\textbf{[TODO]}}}
\newcommand{\shortminus}{\mkern-2mu{\scriptscriptstyle-}\mkern-2mu}
\renewcommand{\arraystretch}{1.3}
% \setlength{\tabcolsep}{.0001\baselineskip} % Adjust horizontal spacing
\DeclareMathOperator{\mean}{mean}
%%%%%
%%%%Hossein 
\usepackage{nicefrac}
\usepackage{lipsum}
% \usepackage{amsfonts, amsthm}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{caption}
\usepackage{subcaption}
% \usepackage{duckuments}

% \usepackage{algorithm, algorithmic}
% \usepackage[hidelinks]{hyperref}
% \ifpdf
%   \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
% \else
%   \DeclareGraphicsExtensions{.eps}
% \fi

% \usepackage{arydshln}
\usepackage{mathtools}
\usepackage{relsize}
\usepackage{booktabs}
% \usepackage{BOONDOX-uprscr}
\usepackage{bm}
% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}


% Change the font size of (a), (b), (c)
% \renewcommand{\subcaplabelfont}{\scriptsize}

% % Change the font size of subfigure captions
% \renewcommand{\subcapsize}{\scriptsize}


% \renewcommand{\thesubfigure}{\scriptsize \alph{subfigure}}  % KEEP THIS


% Used for creating new theorem and remark environments
% \newtheorem{theorem}{Theorem}[section] 
% \newtheorem{definition}{Definition}[section]
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{cor}[theorem]{Corollary}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{assump}[theorem]{Assumption}
% \newtheorem{notation}[theorem]{Notation}
% \newtheorem{example}[theorem]{Example}
% \newtheorem{remark}[theorem]{Remark}
% \newtheorem{claim}[theorem]{Claim}
% Sets running headers as well as PDF title and authors
% \headers{Numerical Method for a non-local diffusive PDE}{D. Do, H. N. Z. Matin and {M. L.} {Delle Monache}}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.


% Authors: full names plus addresses.
% \author{D. Do\thanks{Department of Civil and Environmental Engineering, University of California, Berkeley, California 94720, USA, 
%   (\email{daws@berkley.edu}, \email{h-matin@berkeley.edu}, \email{mldellemonache@berkeley.edu}).}
% \and H. N. Z. Matin\footnotemark[2]
% \and {M. L.} {Delle Monache}\footnotemark[2]}

\usepackage{amsopn}

%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator{\diag}{diag}
\newcommand{\lb}{\left\{}
\newcommand{\rb}{\right\}}
\newcommand{\set}[1]{\left\{ #1 \right \}}
% \newcommand{\loc}{\text{loc}}
\newcommand{\Def}{\overset{\textbf{def}}{=}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\eps}{\varepsilon}
\newcommand{\bOne}{\textcolor{black}{\mathbf{1}}}
\newcommand{\filt}{\mathscr{F}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\uphi}{\underline{\phi}}
% \newcommand{\be}{\mathbf{e}}
\newcommand{\Space}{\mathbf{S}}
\newcommand{\Region}{\mathsf{R}}
\newcommand{\Upper}{\mathsf{U}}
\newcommand{\Lower}{\mathsf{L}}
\newcommand{\la}{\left\langle}
\newcommand{\ra}{\right\rangle}
\newcommand{\bdy}{\partial}
\newcommand{\MID}{\mathcal{T}}
\newcommand{\ff}{\mathbf{f}}
\newcommand{\yy}{\mathfrak{y}}
\newcommand{\Agree}{\mathsf{A}}
\newcommand{\agree}{\mathsf{a}}
\newcommand{\rhomax}{\rho_{\text{max}}}
\newcommand{\fpartial}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\diverg}[1]{\nabla \cdot #1}
\newcommand{\grad}{\nabla}
\newcommand{\alphapos}{\alpha^+}
\newcommand{\alphaneg}{\alpha^-}
\newcommand{\betapos}{\beta^+}
\newcommand{\betaneg}{\beta^-}
\newcommand{\Bv}{\mathbf v}
\newcommand{\Bx}{\mathbf x}
% \newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\abs}[1]{\lvert #1 \rvert}
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\Bu}{\mathbf u}
\newcommand{\Bn}{\mathbf n}
% \newcommand{\Hossein}[1]{\textcolor{teal}{[[Hossein: #1]]}}
\newcommand{\Bz}{\mathbf z}
\newcommand{\upositive}{u^+}
\newcommand{\unegative}{u^-}
% \newcommand{\TV}[1]{\underset{#1}{\text{T.V.}}}
\newcommand{\convex}[1]{\overset{\smallsmile}{#1}}
\newcommand{\concave}[1]{\overset{\smallfrown}{#1}}
\newcommand{\seq}[1]{\left(#1\right)}
\newcommand{\Riemann}{\mathcal R}
\newcommand{\TV}{\textbf{TV}}
\newcommand{\vmax}{\vee}
\newcommand{\wmin}{\wedge}
\newcommand{\sT}{\mathsf T}
\newcommand{\sign}{\text{sign}}
\newcommand{\sx}{\mathsf x}
\newcommand{\front}{\mathfrak D}
\newcommand{\temple}{\mathcal T}
% \newcommand{\zplus}{z^+}
\newcommand{\zminus}{z^-}
\newcommand{\bigmid}{\bigl\vert}
\newcommand{\action}[2]{\langle #1, #2 \rangle}
\newcommand{\tup}[1]{\textup{(}#1\textup{)}}
\usepackage{amsopn}
\newcommand{\totvar}[2]{\underset{#2}{T.V.}\left(#1 \right)}
\newcommand{\BV}{\textbf{BV}}
\DeclareMathOperator{\supp}{Supp}
\DeclareMathOperator{\ball}{Ball}
\DeclareMathOperator{\loc}{loc}
\DeclareMathOperator{\dist}{dist}
\newcommand{\ttilde}[1]{\tilde{\tilde{#1}}}
\newcommand{\sa}{\mathsf a}
\newcommand{\ft}{\mathfrak t}
% \newcommand{\notation}{\textbf{Notation.}}
\newcommand{\pp}{\partial}
\newcommand{\nnorm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}
%%%%%%%%%%%%%%%%
\renewcommand{\vec}[1]{\mathbf #1}
\newcommand{\BX}{\mathbf X}
\newcommand{\kernel}{\mathcal K}
\newcommand{\mapA}{\mathbf{A}}
\newcommand{\timehor}{\mathbf T}
\newcommand{\domain}{\mathfrak D}
\newcommand{\ovmsol}{(\xi_\ell, \xi, \nu_\ell, \nu)}
\newcommand{\By}{\mathbf y}
\newcommand{\Bw}{\mathbf w}
\newcommand{\odelta}{\bar \delta}
\newcommand{\deriv}{\mathscr D}
\newcommand{\cl}{\textbf{cl}}
\newcommand{\topology}{\mathscr T}
\newcommand{\interior}{\textbf{int}}
\newcommand{\Hossein}[1]{\textcolor{teal}{[[Hossein: #1]]}}
\newcommand{\Nathan}[1]{\textcolor{blue}{[[Nathan: #1]]}}


\usepackage{duckuments} % tmp

%%%%%%%%%%%%%%%%%

\usepackage{hyperref}
% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{ifthen}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}
\newsiamremark{fact}{Fact}
\crefname{fact}{Fact}{Facts}
\newsiamthm{case}{Case}


==> q.tex <==
\def \tikzexternallastkey {1233A630277DF80AC2BE1BB390F24C5C}%


==> tex/2d_metrics.tex <==
\begin{table}
    \definecolor{deepcarmine}{rgb}{0.66, 0.13, 0.24}
    \setlength{\tabcolsep}{1pt}
    \centering
    % \scriptsize
        \begin{tabularx}{\textwidth}{c|CCCCC}
        \Xhline{1.pt} 
        & Godunov & WENO & \textbf{NFVM}\(\bm{^1_2}\) & \textbf{NFVM}\(\bm{^5_4}\) & DG\\
        \Xhline{1.pt} 
        Burgers' (L2) & \(1.8\color{deepcarmine}\mathrm{e}^{-3}\)\std{\(6\mathrm{e}^{-4}\)} & \(2.6\color{deepcarmine}\mathrm{e}^{-3}\)\std{\(1\mathrm{e}^{-3}\)} & \(8.3\color{deepcarmine}\mathrm{e}^{-4}\)\std{\(3\mathrm{e}^{-4}\)} & \(2.2\color{deepcarmine}\mathrm{e}^{-4}\)\std{\(1\mathrm{e}^{-4}\)} & \(\bm{1.0}\color{deepcarmine}\bm{\mathrm{e}^{-4}}\)\std{\(4\mathrm{e}^{-5}\)}\\
        Greenshields' (L2) & \(4.1\color{deepcarmine}\mathrm{e}^{-4}\)\std{\(1\mathrm{e}^{-4}\)} & \(6.9\color{deepcarmine}\mathrm{e}^{-4}\)\std{\(4\mathrm{e}^{-4}\)}& \(1.2\color{deepcarmine}\mathrm{e}^{-4}\)\std{\(4\mathrm{e}^{-5}\)} & \(4.6\color{deepcarmine}\mathrm{e}^{-5}\)\std{\(3\mathrm{e}^{-5}\)} & \(\bm{4.2}\color{deepcarmine}\bm{\mathrm{e}^{-5}}\)\std{\(2\mathrm{e}^{-5}\)}\\
        Triangular Sym (L2) & \(2.2\color{deepcarmine}\mathrm{e}^{-3}\)\std{\(1\mathrm{e}^{-3}\)} & \(2.0\color{deepcarmine}\mathrm{e}^{-3}\)\std{\(2\mathrm{e}^{-3}\)} & \(1.3\color{deepcarmine}\mathrm{e}^{-3}\)\std{\(6\mathrm{e}^{-4}\)} & \(2.9\color{deepcarmine}\mathrm{e}^{-4}\)\std{\(2\mathrm{e}^{-4}\)} & \(\bm{2.7}\color{deepcarmine}\bm{\mathrm{e}^{-4}}\)\std{\(1\mathrm{e}^{-4}\)}\\
        \Xhline{1.pt} 
    \end{tabularx}
    \caption{Evaluation of NFVM\(_4^5\) using piecewise constant initial conditions.}
	\label{tab:2d_metrics}
\end{table}

==> tex/default_flow_params.tex <==
% OBSOLETE, now written directly in the main text

\newcolumntype{R}[1]{>{\raggedright\arraybackslash}p{#1}} % left-aligned fixed width

\begingroup
\begin{table}[H]
    \small
    \centering
    \begin{tabularx}{\linewidth}{|R{3.2cm}|C|}
    \hline
        Greenshields' & $v_{\max}=1.0$, $k_{\max}=1.0$ \\
        \hline
        Triangular Sym & $v_{\max}=1.0$, $w=-1.0$, $k_{\max}=1.0$ \\
        \hline
        Triangular Skw & $v_{\max}=2.0$, $w=-1.0$, $k_{\max}=1.0$ \\
        \hline
        Trapezoidal & $v_{\max}=1.0$, $w=-1.5$, $k_{c_1}=0.2$, $k_{c_2}=0.8$, $k_{\max}=1.0$ \\
        \hline
        Greenberg & $c_0=2.0$, $k_{\max}=1.0$ \\
        \hline
        Underwood & $c_1=0.25$, $c_2=1.0$, $k_{\max}=1.0$ \\
        %   Greenshields' & Triangular & Trapezoidal & Greenberg & Underwood\\
        %  $k_{\max}=1.0$ & $k_{\max}=1.0$ & $k_{\max}=1.0$ & $k_{\max}=1.0$ & $k_{\max}=1.0$ \\
        %  $v_{\max}=1.0$ & $v_{\max}=1.0$ & $v_{\max}=1.0$ & $c_0=1.0$ & $c_1=1.0$ \\
        %  & $w=-1.0$ & $w=-1.0$ & & $c_2=2.021$ \\
        % & & $k_{c0} = 0.0118$ & & \\
        % & & $k_{c1} = 0.0404$ & & \\
         \hline
    \end{tabularx}
    \caption{Default parameters for the LWR flow models considered in this work. Values are given in standard units (densities in $\mathrm{veh/m}$, velocities in $\mathrm{m/s}$).}
	\label{tab:default_flow_params}
\end{table}
\endgroup

==> tex/drone_fitted_flows.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[t]{.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/drone_fitted_flows/learnt_greenshields.tikz}
        \captionsetup{labelsep=none, font=scriptsize}
        \subcaption{\thinspace Greenshields'}
    \end{subfigure}
    \begin{subfigure}[t]{.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/drone_fitted_flows/learnt_tri.tikz}
        \captionsetup{labelsep=none, font=scriptsize}
        \subcaption{\thinspace Triangular}
    \end{subfigure}
    \begin{subfigure}[t]{.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/drone_fitted_flows/learnt_trapez.tikz}
        \captionsetup{labelsep=none, font=scriptsize}
        \subcaption{\thinspace Trapezoidal}
    \end{subfigure}
    \begin{subfigure}[t]{.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/drone_fitted_flows/learnt_greenberg.tikz}
        \captionsetup{labelsep=none, font=scriptsize}
        \subcaption{\thinspace Greenberg}
    \end{subfigure}
    \begin{subfigure}[t]{.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/drone_fitted_flows/learnt_underwood.tikz}
        \captionsetup{labelsep=none, font=scriptsize}
        \subcaption{\thinspace Underwood}
    \end{subfigure}
    \caption{\color{red}Fitted flow functions \Nathan{Update these.}}
	\label{fig:drone_fitted_flows}
\end{figure}

==> tex/drone_fitted_heatmaps.tex <==
\begin{figure}
  \centering
  \small
  % GD
  \raisebox{0.61cm}{\rotatebox[origin=c]{90}{GD}}
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/greenshield_godunov_all_heatmap.png}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/triangular_godunov_all_heatmap.png}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/trapezoidal_godunov_all_heatmap.png}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/greenberg_godunov_all_heatmap.png}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/underwood_godunov_all_heatmap.png}
  \end{subfigure}

  % LxF
  \raisebox{0.61cm}{\rotatebox[origin=c]{90}{LxF}}
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/greenshield_lax_friedrichs_all_heatmap.png}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/triangular_lax_friedrichs_all_heatmap.png}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/trapezoidal_lax_friedrichs_all_heatmap.png}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/greenberg_lax_friedrichs_all_heatmap.png}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/underwood_lax_friedrichs_all_heatmap.png}
  \end{subfigure}

  % EO
  \raisebox{0.61cm}{\rotatebox[origin=c]{90}{EO}}
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/greenshield_engquist_osher_all_heatmap.png}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/triangular_engquist_osher_all_heatmap.png}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/trapezoidal_engquist_osher_all_heatmap.png}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/greenberg_engquist_osher_all_heatmap.png}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/underwood_engquist_osher_all_heatmap.png}
  \end{subfigure}

  % ENO
  \raisebox{0.61cm}{\rotatebox[origin=c]{90}{ENO}}
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/greenshield_eno_all_heatmap.png}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/triangular_eno_all_heatmap.png}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/trapezoidal_eno_all_heatmap.png}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/greenberg_eno_all_heatmap.png}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/underwood_eno_all_heatmap.png}
  \end{subfigure}

  % WENO
  \raisebox{0.61cm}{\rotatebox[origin=c]{90}{WENO}}
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/greenshield_weno_all_heatmap.png}
    \vspace{-8.35cm}\caption*{Greenshields'}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/triangular_weno_all_heatmap.png}
    \vspace{-8.35cm}\caption*{Triangular}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/trapezoidal_weno_all_heatmap.png}
    \vspace{-8.35cm}\caption*{Trapezoidal}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/greenberg_weno_all_heatmap.png}
    \vspace{-8.35cm}\caption*{Greenberg}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/drone_fits/underwood_weno_all_heatmap.png}
    \vspace{-8.35cm}\caption*{Underwood}
  \end{subfigure}

  % FLOWS
  % GREENSHIELDS
  \raisebox{0.61cm}{\rotatebox[origin=c]{90}{Flow}}
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    % \includegraphics[width=\textwidth]{figs/drone_fits/underwood_weno_all_heatmap.png}
    \begin{tikzpicture}
        \begin{axis}[
            grid=both,
            only marks, % scatter plot
            width=1.625\linewidth,
            height=1.2\linewidth,
            scaled y ticks=false,
            xtick=\empty,
            ytick=\empty,
            xticklabels=\empty,
            yticklabels=\empty,
          ]
            \addplot[
              mark=*,
              mark size=1pt,
              blue,
              opacity=0.1,
            ] table[
              col sep=comma,
              x expr=\thisrow{density}/4/1609.34,
              y expr=\thisrow{flow}/4/3600
            ] {figs/fundamental_diagram/data_small.csv};
            \addplot[very thick, smooth, color=orange, domain=0:0.10594] {20.009*x*(1.0-x/0.10594)};
          \end{axis}
    \end{tikzpicture}
  \end{subfigure}\hfill
  % TRIANGULAR
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    % \includegraphics[width=\textwidth]{figs/drone_fits/underwood_weno_all_heatmap.png}
    \begin{tikzpicture}
        \begin{axis}[
            grid=both,
            only marks, % scatter plot
            width=1.625\linewidth,
            height=1.2\linewidth,
            scaled y ticks=false,
            xtick=\empty,
            ytick=\empty,
            xticklabels=\empty,
            yticklabels=\empty,
          ]
            \addplot[
              mark=*,
              mark size=1pt,
              blue,
              opacity=0.1,
            ] table[
              col sep=comma,
              x expr=\thisrow{density}/4/1609.34,
              y expr=\thisrow{flow}/4/3600
            ] {figs/fundamental_diagram/data_small.csv};
            \addplot[very thick, smooth, color=orange, domain=0:0.01593] {39.42163*x};
            \addplot[very thick, smooth, color=orange, domain=0.01593:0.152867] {-4.5877 * (x-0.152867)};
          \end{axis}   
    \end{tikzpicture}
  \end{subfigure}\hfill
  % TRAPEZOIDAL
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    % \includegraphics[width=\textwidth]{figs/drone_fits/underwood_weno_all_heatmap.png}
    \begin{tikzpicture}
        \begin{axis}[
            grid=both,
            only marks, % scatter plot
            width=1.625\linewidth,
            height=1.2\linewidth,
            scaled y ticks=false,
            xtick=\empty,
            ytick=\empty,
            xticklabels=\empty,
            yticklabels=\empty,
          ]
            \addplot[
              mark=*,
              mark size=1pt,
              blue,
              opacity=0.1,
            ] table[
              col sep=comma,
              x expr=\thisrow{density}/4/1609.34,
              y expr=\thisrow{flow}/4/3600
            ] {figs/fundamental_diagram/data_small.csv};
            \addplot[very thick, smooth, color=orange, domain=0:0.0118300] {39.4904236*x};
            \addplot[very thick, smooth, color=orange, domain=0.0118300:0.04041] {0.467171 + (x - 0.0118300) * (0.467171 - 0.467171)/(0.0118300 - 0.040417)};
            \addplot[very thick, smooth, color=orange, domain=0.04041:0.142490] {-4.576839560 * (x-0.1424900)};
          \end{axis}   
    \end{tikzpicture}
  \end{subfigure}\hfill
  % GREENBERG
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    % \includegraphics[width=\textwidth]{figs/drone_fits/underwood_weno_all_heatmap.png}
    \begin{tikzpicture}
        \begin{axis}[
            grid=both,
            only marks, % scatter plot
            width=1.625\linewidth,
            height=1.2\linewidth,
            scaled y ticks=false,
            xtick=\empty,
            ytick=\empty,
            xticklabels=\empty,
            yticklabels=\empty,
          ]
            \addplot[
              mark=*,
              mark size=1pt,
              blue,
              opacity=0.1,
            ] table[
              col sep=comma,
              x expr=\thisrow{density}/4/1609.34,
              y expr=\thisrow{flow}/4/3600
            ] {figs/fundamental_diagram/data_small.csv};
            \addplot[very thick, smooth, color=orange, domain=0:0.106515] {7.0944226454 * x * ln(0.10651502/(x + 1e-7))};
          \end{axis}   
    \end{tikzpicture}
  \end{subfigure}\hfill
  % UNDERWOOD
  \begin{subfigure}[t]{.193\textwidth}
    \centering
    % \includegraphics[width=\textwidth]{figs/drone_fits/underwood_weno_all_heatmap.png}
    \begin{tikzpicture}
        \begin{axis}[
            grid=both,
            only marks, % scatter plot
            width=1.625\linewidth,
            height=1.2\linewidth,
            scaled y ticks=false,
            xtick=\empty,
            ytick=\empty,
            xticklabels=\empty,
            yticklabels=\empty,
          ]
            \addplot[
              mark=*,
              mark size=1pt,
              blue,
              opacity=0.1,
            ] table[
              col sep=comma,
              x expr=\thisrow{density}/4/1609.34,
              y expr=\thisrow{flow}/4/3600
            ] {figs/fundamental_diagram/data_small.csv};
            \addplot[very thick, smooth, color=orange, domain=0:0.15] {0.68371646 * exp(1) * x * exp(-2.021423 * x)};
            % \addplot[very thick, smooth, color=orange, domain=0:0.2486144] {0.68371646 * exp(1) * x * exp(-2.021423 * x)};
          \end{axis}
    \end{tikzpicture}
  \end{subfigure}

  \caption{Forward prediction over the whole dataset using all fitted FVMs on considered traffic flows. The axes and colorbars are the same for all heatmap plots, and are identical as in~\Cref{fig:drone_dataset_heatmap}. For the last row of plots, the axes are the same as in~\Cref{fig:fundamental_diagram}. (Note: the flows are calibrated on the prediction, not on the cloud points!)}
  \label{fig:drone_fitted_heatmaps}
\end{figure}

==> tex/drone_fitted_heatmaps_train.tex <==
\begin{figure}
    \centering
    \small
    \begin{subfigure}[t]{.193\textwidth}
      \centering
      \includegraphics[width=\textwidth]{figs/drone_fits/greenshield_godunov_train_heatmap.png}
      \caption*{Greenshields'}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{.193\textwidth}
      \centering
      \includegraphics[width=\textwidth]{figs/drone_fits/triangular_godunov_train_heatmap.png}
      \caption*{Triangular}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{.193\textwidth}
      \centering
      \includegraphics[width=\textwidth]{figs/drone_fits/trapezoidal_godunov_train_heatmap.png}
      \caption*{Trapezoidal}  
    \end{subfigure}\hfill
    \begin{subfigure}[t]{.193\textwidth}
      \centering
      \includegraphics[width=\textwidth]{figs/drone_fits/greenberg_godunov_train_heatmap.png}
      \caption*{Greenberg}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{.193\textwidth}
      \centering
      \includegraphics[width=\textwidth]{figs/drone_fits/underwood_godunov_train_heatmap.png}
      \caption*{Underwood}
    \end{subfigure}
  
    \caption{Forward prediction on the training set, on which the flows are fitted.}
    \label{fig:drone_fitted_heatmaps_train}
\end{figure}

==> tex/drone_fitted_params.tex <==
% OBSOLETE, now drone_fitted_fd.tex

% \begingroup
% \begin{table}[H]
%     \small
%     \centering
%     \begin{tabularx}{\linewidth}{CCCCC}
%     \hline
%          \Xhline{1.pt} 
%           Greenshields' & Triangular & Trapezoidal & Greenberg & Underwood\\
%          \Xhline{1.pt} 
%          $k_{\max}=0.106$ & $k_{\max}=0.153$ & $k_{\max}=0.142$ & $k_{\max}=0.107$ & $k_{\max}=0.249$ \\
%          $v_{\max}=20.01$ & $v_{\max}=39.42$ & $v_{\max}=39.49$ & $c_0=7.09$ & $c_1=0.684$ \\
%          & $w=-4.58$ & $w=-4.57$ & & $c_2=2.021$ \\
%         & & $k_{c_1} = 0.0118$ & & \\
%         & & $k_{c_2} = 0.0404$ & & \\
%          \Xhline{1.pt} 
%     \end{tabularx}
%     \caption{Fitted parameters for the flows calibrated on the drone dataset (see~\Cref{fig:drone_fitted_heatmaps}). Values are given in standard units (densities in $\mathrm{veh/m}$, velocities in $\mathrm{m/s}$).}
% 	\label{tab:drone_fitted_params}
% \end{table}
% \endgroup

==> tex/drone_l2_errors.tex <==
\begingroup
\setlength{\tabcolsep}{2pt}
\begin{table}[H]
    \centering
    \begin{tabularx}{\linewidth}{c||CCCCC||CC}
    \hline
         \Xhline{1.pt} 
         & GD & LxF & EO & ENO & WENO & NN 1D & NN 2D \\
         \Xhline{1.pt} 
            Greenshields' & \(5.14\mathrm{e}^{-2}\) & \(4.54\mathrm{e}^{-2}\) & \(5.14\mathrm{e}^{-2}\) & \(1.75\mathrm{e}^{-1}\) & \(4.74\mathrm{e}^{-2}\) %
            &  \multirow{5}{*}{\(\bm{1.63\mathrm{e}^{-2}}\)} & \multirow{5}{*}{\(\bm{1.54\mathrm{e}^{-2}}\)} \\
            Triangular & \(2.06\mathrm{e}^{-2}\) & \(1.88\mathrm{e}^{-2}\) & \(2.79\mathrm{e}^{-2}\) & \(2.37\mathrm{e}^{-2}\) & \(1.85\mathrm{e}^{-2}\) %
            & & \\
            Trapezoidal & \(4.49\mathrm{e}^{-2}\) & \(3.89\mathrm{e}^{-2}\) & \(4.49\mathrm{e}^{-2}\) & \(1.29\mathrm{e}^{-1}\) & \(4.04\mathrm{e}^{-2}\) %
            & & \\
            Greenberg & \(6.20\mathrm{e}^{-2}\) & \(5.13\mathrm{e}^{-2}\) & \(6.72\mathrm{e}^{-2}\) & \(7.93\mathrm{e}^{-2}\) & \(3.89\mathrm{e}^{-2}\) %
            & & \\
            Underwood & \(4.88\mathrm{e}^{-2}\) & \(4.33\mathrm{e}^{-2}\) & \(4.89\mathrm{e}^{-2}\) & \(3.04\mathrm{e}^{-1}\) & \(3.88\mathrm{e}^{-2}\) %
            & & \\
         \Xhline{1.pt} 
    \end{tabularx}
    \caption{L2 errors of the forward prediction over the whole dataset using all fitted FVMs on considered traffic flows, as well as the trained NFVM models. \Nathan{Update these if we decide to keep them.}}
	\label{tab:drone_l2_errors}
\end{table}
\endgroup

